The ADMM penalized decoder for LDPC codes

Linear programming (LP) decoding for low-density parity-check (LDPC) codes proposed by Feldman et al. is shown to have theoretical guarantees in several regimes and empirically is not observed to suffer from an error floor. However at low signal-to-noise ratios (SNRs), LP decoding is observed to have worse error performance than belief propagation (BP) decoding. In this paper, we seek to improve LP decoding at low SNRs while still achieving good high SNR performance. We first present a new decoding framework obtained by trying to solve a non-convex optimization problem using the alternating direction method of multipliers (ADMM). This non-convex problem is constructed by adding a penalty term to the LP decoding objective. The goal of the penalty term is to make "pseudocodewords", which are the non-integer vertices of the LP relaxation to which the LP decoder fails, more costly. We name this decoder class the "ADMM penalized decoder". In our simulation results, the ADMM penalized decoder with $\ell_1$ and $\ell_2$ penalties outperforms both BP and LP decoding at all SNRs. For high SNR regimes where it is infeasible to simulate, we use an instanton analysis and show that the ADMM penalized decoder has better high SNR performance than BP decoding. We also develop a reweighted LP decoder using linear approximations to the objective with an $\ell_1$ penalty. We show that this decoder has an improved theoretical recovery threshold compared to LP decoding. In addition, we show that the empirical gain of the reweighted LP decoder is significant at low SNRs.

==> sec_simulation.tex <==
\section{Numerical results}
\label{sec.numerical}
In this section, we present numerical results for \pPDn. 
In Section~\ref{sec.sim.wer}, we present word-error-rate (WER) comparisons
among \pPD using $\ell_1$ and $\ell_2$ penalty and other decoders (BP and LP). 
We do not present simulation results for \pRLP because it is not the best
performing decoder. We refer to~\cite{liu2012the} for readers interested in performance
of \pRLPn.
In Section~\ref{sec.sim.parameter}, we study the effect of choosing
different parameters. We show that even though the parameter search
space is large, it is easy to obtain high performing parameter set.
In Section~\ref{sec.sim.instanton}, we present instanton analysis for 
\pPDn. We show instanton profile of the $[155,64]$ Tanner code~\cite{tanner2001class} and weaknesses
for \pPDn. Further, we demonstrate that the predictions made by instantons
for \pPD with $\ell_2$ penalty are accurate at high SNRs.

\subsection{WER performance}
\label{sec.sim.wer}
We simulate the $[2640,1320]$ ``Margulis''
code~\cite{ryanlin2009channel} for an AWGN channel with the following parameter 
settings: $\mu = 3$, $\epsilon = 10^{-5}$ and maximum number of iterations 
$T_{\max} = 1000$. For $\ell_1$ and $\ell_2$ penalty, we pick $\alpha_1 = 0.6$
$\alpha_2 = 0.8$ respectively (cf.~\eqref{eq.lpl1penalty}
and \eqref{eq.lpl2penalty}). We defer discussion for optimal parameter to
Section~\ref{sec.sim.parameter} and Section~\ref{sec.sim.instanton}. 
\begin{figure}[h]
\psfrag{&ADMMLP}{\scriptsize{ADMM LP decoding}}
\psfrag{&BPSaturation}{\scriptsize{BP decoding (Ryan and Lin)}}
\psfrag{&BPNonSat}{\scriptsize{Non-saturating BP decoding}}
\psfrag{&ADMM-L1PenaliedDecoder}{\scriptsize{\pPD with $\ell_1$ penalty }}
\psfrag{&ADMM-L2PenaliedDecoder}{\scriptsize{\pPD with $\ell_2$ penalty }}
\psfrag{&SNR}{\scriptsize{\hspace{-1mm}$E_b/N_0(dB)$}}
\psfrag{&WER}{\scriptsize{WER}}

\psfrag{1}{\scriptsize{$1$}}
\psfrag{1.5}{\scriptsize{$1.5$}}
\psfrag{2}{\scriptsize{$2$}}
\psfrag{2.5}{\scriptsize{$2.5$}}
\psfrag{3}{\scriptsize{$3$}}


\psfrag{10}{\scriptsize{\hspace{-1mm}$10$}}
\psfrag{-2}{\tiny{\hspace{-1mm}$-2$}}
\psfrag{-4}{\tiny{\hspace{-1mm}$-4$}}
\psfrag{-6}{\tiny{\hspace{-1mm}$-6$}}
\psfrag{-8}{\tiny{\hspace{-1mm}$-8$}}

\psfrag{e0}{\tiny{\hspace{-1mm}$0$}}

    \begin{center}
    \includegraphics[width=9.5cm]{figures/MargulisCodeAWGN.eps}
    \end{center}
    \caption{Word-error-rate (WER) vs. $E_b / N_0$ performance for the
      $[2640,1320]$ ``Margulis'' code.}
    \label{fig.sim_margulis}
\end{figure}
In Fig.~\ref{fig.sim_margulis}, we
plot the WER as a function of SNR. For each data point, we also plot
the error bar. Data for BP and LP decoder are drawn from~\cite{barman2013decomposition}.
For $E_b/N_0 = 2.3dB, 2.4dB$, we collect $43$ and $13$ respective errors for 
\pPD with $\ell_1$ penalty. For $E_b/N_0 = 2.5dB$, we collect $9$ errors for \pPD with $\ell_2$ penalty.
All other data points are based on more than $200$ errors.

Recall from Section
~\ref{sec.introduction} that the
``non-saturating BP'' is a robust BP implementation that avoids
saturating the log-likelihood ratios of the sum-product BP decoder, thereby improving decoding
performance in the error floor regime. We note, again, that LP decoding
performs worse than non-saturating BP decoding at low SNRs. However
LP decoding shows better high SNR trend. The WER of \pPD combines the good characteristics of both LP and
BP decoders: The decoders that uses the $\ell_1$ and $\ell_2$ penalty
function both perform as well as BP decoder at low SNRs. In addition,
the slope of the WER curves of both decoders continue to
increase at WERs around $10^{-9}$.  This is similar to LP decoder. We observe
that \pPD runs faster than our baseline sum-product
BP implementation. We also note that decoding using the $\ell_2$
penalty has the best error performance and time efficiency among the
three penalty functions presented. Thus, we consider the decoder that
uses the $\ell_2$ penalty to be a strong competitor to the classic BP
algorithm.

It is worth mentioning that WER for \pPD using $\ell_2$ penalty tends to
be a straight line at $E_b/N_0= 2.5dB$. This high SNR behavior is further 
studied and discussed in Section~\ref{sec.sim.instanton}, where we 
show that best parameter $\alpha$ should be small for high SNRs. Due to 
limited computational resources we did not simulate other $\alpha$'s for
high SNRs.

\begin{figure}[h]
\psfrag{&ADMMLP}{\scriptsize{ADMM LP decoding}}
\psfrag{&BPNonSat}{\scriptsize{Non-saturating BP decoding}}
\psfrag{&ADMM-L1PenaliedDecoder}{\scriptsize{\pPD with $\ell_1$ penalty }}
\psfrag{&ADMM-L2PenaliedDecoder}{\scriptsize{\pPD with $\ell_2$ penalty }}
\psfrag{&SNR}{\scriptsize{\hspace{-1mm}$E_b/N_0(dB)$}}
\psfrag{&WER}{\scriptsize{WER}}

\psfrag{1}{\scriptsize{$1$}}
\psfrag{1.2}{\scriptsize{$1.2$}}
\psfrag{1.4}{\scriptsize{$1.4$}}
\psfrag{1.6}{\scriptsize{$1.6$}}
\psfrag{1.8}{\scriptsize{$1.8$}}
\psfrag{2}{\scriptsize{$2$}}
\psfrag{2.2}{\scriptsize{$2.2$}}
\psfrag{2.4}{\scriptsize{$2.4$}}
\psfrag{2.6}{\scriptsize{$2.6$}}

\psfrag{10}{\scriptsize{\hspace{-1mm}$10$}}
\psfrag{-2}{\tiny{\hspace{-1mm}$-2$}}
\psfrag{-4}{\tiny{\hspace{-1mm}$-4$}}
\psfrag{-6}{\tiny{\hspace{-1mm}$-6$}}
\psfrag{-8}{\tiny{\hspace{-1mm}$-8$}}

\psfrag{e0}{\tiny{\hspace{-1mm}$0$}}

    \begin{center}
    \includegraphics[width=9.5cm]{figures/MackayCodeAWGN.eps}
    \end{center}
    \caption{Word-error-rate (WER) vs. $E_b / N_0$ performance for the
      Mackay 12398 code.}
    \label{fig.sim_mackay}
\end{figure}

In Fig.~\ref{fig.sim_mackay}, we plot the WER performance for a long block length code obtained 
from~\cite{Database}. All data points are based on more than $200$ decoding errors.
This code has length $12398$ and rate $0.25$. Compared 
to the Margulis code, this code is significantly longer. 
 The decoder parameter settings are the same as the previous 
experiment. We did not further optimize parameter settings 
for this code due to limited computational resources. Further,
as shown in Fig.~\ref{fig.sim_mackay}, these parameters already 
perform well. We observe from Fig.~\ref{fig.sim_mackay}
that LP decoding suffers from significant SNR degradation compared to sum-product BP decoding.
\pPD decoders shrink the SNR gap between BP and LP decoding by approximately $0.8dB$. Further,
\pPD keeps the good high SNRs trending from LP decoding. The WER slope for \pPD
at $E_b/N_0 = 1.5, 1.6dB$ is steeper than that for BP decoding. 

To summarize, \pPD displays best error performance for the code and SNR we simulate.
What is more, \pPD is also the fastest among the decoders we simulated. These make
\pPD a very strong competitor among the decoders studied in this work.


\subsection{Choice of parameters}
\label{sec.sim.parameter}
There are many parameters for \pPD. As a reminder, these parameters include:
penalty term coefficient $\alpha$, ADMM augmented Lagrangian weight $\mu$, 
ADMM ending tolerance $\epsilon$, ADMM maximum number of iterations $T_{\max}$
and ADMM over-relaxation parameter $\rho$ (cf.~\cite{barman2013decomposition}). The optimal parameter settings
depend on the both the code and SNR. Exhaustively 
search for all possible combinations of parameters for all SNRs is infeasible and
is not the focus of this paper. The parameter choice principles learned in this paper 
is already satisfactory in order to obtain good performances as demonstrated in Section~\ref{sec.sim.wer}.
In this section, 
we search for optimal parameters via simulation for low SNRs. We fix some parameters
and then search for the rest. In Section~\ref{sec.sim.instanton}, we use instanton to argue parameter
choices at high SNRs where simulation based searching is infeasible.

We first study WER as a function of $\alpha_i, i \in\{1,2\}$ for
the respective updates steps of~\eqref{eq.lpl1penalty}
and \eqref{eq.lpl2penalty} in
Fig.~\ref{fig.sim_margulis_parameteralpha_snr_wer} 
and
Fig.~\ref{fig.sim_margulis_parameteralpha_other_wer}. 
 We fix the ADMM parameters $\mu = 3$, $\epsilon = 10^{-5}$.
  For each data point, we collect more than
$200$ errors. 
In Fig.~\ref{fig.sim_margulis_parameteralpha_snr_wer}, we fix the maximum number
of iterations $T_{\max} = 1000$. In Fig.~\ref{fig.sim_margulis_parameteralpha_other_wer}, we only plot data for 
\pPD with $\ell_2$ penalty for conciseness. The respective bahavior for $\ell_1$ penalty is 
similar to Fig.~\ref{fig.sim_margulis_parameteralpha_other_wer}.

\begin{figure}
\psfrag{&&&&L1PenaliedDecoderSNR16}{\scriptsize{$\ell_1$ penalty, $E_b/N_0 = 1.6dB$}}
\psfrag{&&&&L2PenaliedDecoderSNR16}{\scriptsize{$\ell_2$ penalty, $E_b/N_0 = 1.6dB$}}
\psfrag{&&&&L1PenaliedDecoderSNR19}{\scriptsize{$\ell_1$ penalty, $E_b/N_0 = 1.9dB$}}
\psfrag{&&&&L2PenaliedDecoderSNR19}{\scriptsize{$\ell_2$ penalty, $E_b/N_0 = 1.9dB$}}
\psfrag{&Alpha}{\scriptsize{$\alpha_i$; $i = \{1,2\}$}}
\psfrag{&WER}{\scriptsize{WER}}

\psfrag{0}{\scriptsize{$0$}}
\psfrag{1}{\scriptsize{$1$}}
\psfrag{2}{\scriptsize{$2$}}
\psfrag{3}{\scriptsize{$3$}}
\psfrag{4}{\scriptsize{$4$}}
\psfrag{5}{\scriptsize{$5$}}
\psfrag{6}{\scriptsize{$6$}}
\psfrag{10}{\scriptsize{\hspace{-1mm}$10$}}
\psfrag{-1}{\tiny{\hspace{-1mm}$-1$}}
\psfrag{e0}{\tiny{\hspace{-1mm}$0$}}
    \begin{center}
    \includegraphics[width=9.25cm]{figures/ParameterAlpha_SNR.eps}
    \end{center}
    \caption{Word-error-rate (WER) of the $[2640,1320]$ ``Margulis'' code for the AWGN channel plotted as a function of the choice of $\alpha_i$; $E_b/N_0 = 1.6dB$ and $1.9dB$.}
    \label{fig.sim_margulis_parameteralpha_snr_wer}
\end{figure}

\begin{figure}
\psfrag{&&&&Tmax200Overrel1}{\scriptsize{$T_{\max} = 200$, $\rho = 1$}}
\psfrag{&&&&Tmax200Overrel19}{\scriptsize{$T_{\max} = 200$, $\rho = 1.9$}}
\psfrag{&&&&Tmax1000Overrel1}{\scriptsize{$T_{\max} = 1000$, $\rho = 1$}}
\psfrag{&&&&Tmax1000Overrel19}{\scriptsize{$T_{\max} = 1000$, $\rho = 1.9$}}
\psfrag{&Alpha}{\scriptsize{$\alpha_i$; $i = \{1,2\}$}}
\psfrag{&WER}{\scriptsize{WER}}

    \begin{center}
    \includegraphics[width=9.25cm]{figures/ParameterAlpha_IterOverrel.eps}
    \end{center}
    \caption{Word-error-rate (WER) of the $[2640,1320]$ ``Margulis'' code for the AWGN channel plotted as a function of the choice of $\alpha_i$; $E_b/N_0 = 1.6dB$ with different maximum number of iterations $T_{\max}$ and over-relaxation parameter $\rho$. \pPD with $\ell_2$ penalty.}
    \label{fig.sim_margulis_parameteralpha_other_wer}
\end{figure}

We make the following observations: First, the WER drops quickly as we start to penalize
fractional solutions (increasing the $\alpha_i$ above
zero). But the WER increases
when we penalize too heavily, e.g., when $\alpha_1>0.5, \alpha_2>0.8$. 
The WERs then slowly increase again up to unity. The
globally optimal parameter choices are $\alpha_1^* = 0.5, \alpha_2^* =
0.8$. Second, the optimal parameters are almost the same for $E_b/N_0 = 1.6$ and $1.9dB$.
Recall that in Fig.~\ref{fig.sim_margulis}, we used the same $\alpha$'s in all SNRs and 
received consistent gains throughout all SNRs. Although this simplifies practical implementation,
one needs to be careful at high SNRs. We defer detailed discussions to Section~\ref{sec.sim.instanton}
Third, although different values for
$T_{\max}$ give almost the same performance for LP decoding (see
points at $\alpha_i = 0$), $T_{\max}$ does affect the performance when
a penalty term is added. We see from
Fig.~\ref{fig.sim_margulis_parameteralpha_other_wer} that when more iterations
are allowed, the WER decreases substantially. Similar argument also applies to the
over-relaxation parameter. Note that when $\rho = 1.9$, $\alpha_1^*$ becomes $0.6$.

In Fig.~\ref{fig.sim_margulis_parametermu_other_wer}, we focus on parameter $\mu$ and study
its effect on WER. We observe that the WER has some weak dependencies on $\mu$. The optimal $\mu$'s for
$T_{\max} = 200$ and $T_{\max} = 1000$ are $\mu = 4$ and $\mu = 3$ respectively. In fact, even
if the decoder is not operating on the best $\mu$, the performance has little degradation. We
also note that the decoding time for different $\mu$ changes little for $\mu \in [2,6]$ (data not
shown here). Thus we conclude that parameter $\mu$ has smaller impact to the decoder compared to
parameter $\alpha$. This property provides rich choices for $\mu$ in practice.

\begin{figure}
\psfrag{&&&&&L1Tmax200Overrel1}{\scriptsize{$T_{\max} = 200$, $\ell_1$ penalty}}
\psfrag{&&&&&L2Tmax200Overrel1}{\scriptsize{$T_{\max} = 200$, $\ell_2$ penalty}}
\psfrag{&&&&&L1Tmax1000Overrel1}{\scriptsize{$T_{\max} = 1000$, $\ell_1$ penalty}}
\psfrag{&&&&&L2Tmax1000Overrel1}{\scriptsize{$T_{\max} = 1000$, $\ell_2$ penalty}}
\psfrag{&Mu}{\scriptsize{$\mu$}}
\psfrag{&WER}{\scriptsize{WER}}

    \begin{center}
    \includegraphics[width=9.25cm]{figures/ParameterMu_IterOverrel.eps}
    \end{center}
    \caption{Word-error-rate (WER) of the $[2640,1320]$ ``Margulis'' code for the AWGN channel plotted as a function of the choice of $\mu$; $E_b/N_0 = 1.6dB$ with different maximum number of iterations $T_{\max}$.}
    \label{fig.sim_margulis_parametermu_other_wer}
\end{figure}

In Fig.~\ref{fig.sim_margulis_parameteralpha_snr_iter}, we study effects of parameter $\alpha$
on decoder complexity. We make three remarks: First, the best parameter choice in terms of
WER agrees with the best parameter choice in terms of complexity. In particular, note that data in
 Fig.~\ref{fig.sim_margulis_parameteralpha_snr_iter} is for correct decoding events. If 
 we were to plot \textbf{average} number of iterations, the best WER choice 
($\alpha_1 = 0.5$ and $\alpha_2 = 0.8$ from Fig.~\ref{fig.sim_margulis_parameteralpha_snr_wer}) is more likely to 
 display best decoder complexity due to the fact that erroneous events consumes much more iterations.
Second, the number of iterations required is much smaller than ADMM LP decoder (points where $\alpha_i = 0$ for $i = 1,2$).
We recall the results in~\cite{barman2012decomposition} that decoding time for ADMM LP decoder 
is comparable to BP decoder. In recent works~\cite{zhang2013large, zhang2013efficient}, the author proposed improvement to projection
algorithm, which can benefit \pPD as well. Thus we expect that \pPD to be a strong competitor against
BP decoding in terms of decoding complexity. 
\begin{figure}
\psfrag{&ADML1IterationsCorrectSNR16}{\scriptsize{$\ell_1$ penalty, $E_b/N_0 = 1.6dB$}}
\psfrag{&ADML2IterationsCorrectSNR16}{\scriptsize{$\ell_2$ penalty, $E_b/N_0 = 1.6dB$}}
\psfrag{&ADML1IterationsCorrectSNR19}{\scriptsize{$\ell_1$ penalty, $E_b/N_0 = 1.9dB$}}
\psfrag{&ADML2IterationsCorrectSNR19}{\scriptsize{$\ell_2$ penalty, $E_b/N_0 = 1.9dB$}}
\psfrag{&Alpha}{\scriptsize{$\alpha_i$; $i = \{1,2\}$}}
\psfrag{&Iteration}{\scriptsize{\# Iteration}}

    \begin{center}
    \includegraphics[width=9.25cm]{figures/ParameterAlphaIteration_SNR.eps}
    \end{center}
    \caption{Number of iterations of \textbf{correct decoding events} of the $[2640,1320]$ ``Margulis'' code for the AWGN channel plotted as a function of the choice of $\alpha_i$; $E_b/N_0 = 1.6dB$ and $1.9dB$.}
    \label{fig.sim_margulis_parameteralpha_snr_iter}
\end{figure}


We summarize the parameter choices learned in this section: $\alpha_1 = 0.6$ and $\alpha_2 = 0.8$ are good choices for $\ell_1$ and $\ell_2$ penalties respectively; $\mu \in [3,5]$ are all good choices for both penalty choices; large $T_{\max}$ improves WER performance at cost of computation complexity; $\rho = 1.9$ is best for both WER and decoder speed. We do not present data for parameter $\epsilon$, but we note that $\epsilon < 10^{-5}$ is good for both WER and decoder speed.

\iffalse
\begin{figure}
\psfrag{&L1ExecutionTimeCorrectSNR16}{\scriptsize{$\ell_1$ penalty, $E_b/N_0 = 1.6dB$}}
\psfrag{&L2ExecutionTimeCorrectSNR16}{\scriptsize{$\ell_2$ penalty, $E_b/N_0 = 1.6dB$}}
\psfrag{&L1ExecutionTimeCorrectSNR19}{\scriptsize{$\ell_1$ penalty, $E_b/N_0 = 1.9dB$}}
\psfrag{&L2ExecutionTimeCorrectSNR19}{\scriptsize{$\ell_2$ penalty, $E_b/N_0 = 1.9dB$}}
\psfrag{&Alpha}{\scriptsize{$\alpha_i$; $i = \{1,2\}$}}
\psfrag{&exeTime}{\scriptsize{Execution Time (sec)}}

    \begin{center}
    \includegraphics[width=9.25cm]{figures/ParameterAlphaTime_SNR.eps}
    \end{center}
    \caption{Decoding time of \textbf{correct decoding events} of the $[2640,1320]$ ``Margulis'' code for the AWGN channel plotted as a function of the choice of $\alpha_i$; $E_b/N_0 = 1.6dB$ and $1.9dB$.}
    \label{fig.sim_margulis_parameteralpha_snr_time}
\end{figure}
\fi
\subsection{Instanton profile for the $[155,64]$ code}
\label{sec.sim.instanton}
We study the instantons for the $[155,64]$ code and use the results to predict high SNR WER. We note that from previous results, we have seen that 
the $\ell_2$ penalty achieves the best performance in terms of both error rate and decoding complexity,
making it a preferred candidate in practice. Thus we focus on the $\ell_2$ norm penalty in this section
to obtain instanton information.

In Figure~\ref{fig.inst_norm}, we plot the minimum instanton norm as a function of penalty coefficient $\alpha_2$. We fix parameters as follows:
$\mu = 3$, $T_{\max} = 1000$, $\rho = 1.9$, $\epsilon = 10^{-5}$.
When the penalty coefficient is $0$, the decoder becomes an LP decoder. The minimum instanton norm matches the result in~\cite{chertkov2008efficient}. As we start to penalize the objective, we see that there is a clear trend that as the penalty increases, the minimum instanton norm decreases.
This implies that when we put more penalty on pseudocodewords, we get worse performance at high SNRs. Instanton information in Fig.~\ref{fig.inst_norm} can be used to predict decoder performance at high SNRs similar to those exist in the literature (e.g.~\cite{stepanov2005diagnosis}). In Fig.~\ref{fig.sim_15564_instanton}, we plot the WER predicted by minimum norm instanton as well as real simulation results. We make two observations: First, the instanton norm predicts simulation outcome very nicely for this code. Second, there exist a crossover point where LP decoding outperforms \pPDn. This matches our expectation from instanton results in Fig.~\ref{fig.inst_norm}. 

These results are important because of two reasons. First, this shows that although \pPD outperforms LP decoder in Fig~\ref{fig.sim_margulis} and Fig~\ref{fig.sim_mackay}, it is not as good as LP decoder at high SNRs asymptotically for nonzero penalty coefficients. Second, in practice, we need to adjust the penalty parameter according to different SNRs the code operates at. In particular, we can expect that small penalty coefficient produces better error rate performance at high SNRs as shown in Fig.~\ref{fig.sim_15564_instanton}.

We also observe from Fig.~\ref{fig.inst_norm} that the instanton data for large penalty coefficient ($\alpha > 1.5$) behaves more chaotic than small penalty coefficients ($\alpha < 1$). The authors believe that this is because of the non-convexity nature of \pPD. However, we note that the coefficient we are interested in are usually small (cf. Section~\ref{sec.sim.parameter}), making this behavior less important. On the other hand, one may get better data for small number of iterations or use some DFO techniques such as Nelder Mead method \cite{nocedal2006numerical} or Nesterov's gradient free \cite{nesterov2011random} as a refine step after getting initial output from Algorithm~\ref{Algorithm.instanton}. 
\begin{figure}
\psfrag{&A}{\scriptsize{\hspace{-1cm} penalty parameter $\alpha_2$}}
\psfrag{&B}{\scriptsize{\hspace{-1cm} Minimum instanton norm}}
	\begin{center}
    \includegraphics[width=9.5cm]{figures/minimum_instanton_norm.eps}
    \end{center}
    \caption{Minimum instanton norm as a function of penalty parameter for the
      $[155,64]$ code when decoded with \pPD with $\ell_2$ penalty.}
    \label{fig.inst_norm}
\end{figure}


\begin{figure}[h]
\psfrag{&ADMMLP}{\scriptsize{ADMM LP decoding}}
\psfrag{&ADMML2}{\scriptsize{\pPD with $\ell_2$ penalty}}
\psfrag{&InstantonPredictionForL2-padpadpadpadpad}{\scriptsize{Prediction by instanton at $\alpha_2 = 2$}}
\psfrag{&InstantonPredictionForLP}{\scriptsize{Prediction by pseudocodewords for LP}}
\psfrag{&SNR}{\scriptsize{\hspace{-1mm}$E_b/N_0(dB)$}}
\psfrag{&WER}{\scriptsize{WER}}
\begin{center}
\includegraphics[width=8cm]{figures/InstantonSimulation.eps}
\end{center}
\caption{Simulation vs. instanton predictions for $[155,64]$ code.}
\label{fig.inst_sim}
\end{figure}

In Figure~\ref{fig.sim_15564_instanton}, we further investigate the failure events for \pPDn. 
We observe that for minimum norm instantons, most bits are zero while there are only a few nonzero entries. Moreover, these nonzero entries are
related to trapping set structure. As an example, we show one minimum instanton for $\alpha = 0.9$. 
For the non-zero entries, we select the 5 entries with the largest value and found that these 5 bits are in a (5,3) trapping set (shown in Figure~\ref{fig.sim_15564_instanton}). This effect is similar to other sub-optimal decoders (BP and LP)~\cite{chilappagari2009instanton}. One can expect that code designs that alleviate trapping set effect can also benefit ~\pPDn.

\begin{figure}[h]
\begin{center}
\includegraphics[width=8cm]{figures/trappingset.eps}
\end{center}
\caption{Topology of (5,3) trapping set, each node indexed by the variable or check number.}
\label{fig.sim_15564_instanton}
\end{figure}
